Fermion pair production in e+e- collisions at 189-209 GeV and constraints on physics beyond the Standard Model

Cross sections, angular distributions and forward-backward asymmetries are presented, of two-fermion events produced in e+e- collisions at centre-of-mass energies from 189 to 209 GeV at LEP, measured with the ALEPH detector. Results for e+e-, mu+mu-, tau+tau-, qq, bb and cc production are in agreement with the Standard Model predictions. Constraints are set on scenarios of new physics such as four-fermion contact interactions, leptoquarks, Z' bosons, TeV-scale quantum gravity and R-parity violating squarks and sneutrinos.

==> tab-afbb-syst.tex <==
%Afbb Systematics
\begin{table}[hbtp]
\centering
  \caption{\label{tab:afbb-syst}{\small {Contributions to the systematic
  uncertainties on the measured values of 
  ${A_{\rm FB}^{\rm b}}$  over the angular range $|\cos\theta|<0.9$,
   as a function of the centre-of-mass energy. }} }
  \vspace*{0.5cm}
  \begin{center}
    \begin{tabular}{|l|ccccccc|}
      \hline
      Source & \multicolumn{7}{c|}{${E_{\rm cm}}$ (GeV) } \\
      & 189 & 192 & 196 & 200 & 202 & 205 & 207 \\

      \hline
      MC statistics           & 0.0051 & 0.0077 & 0.0045 & 0.0080 & 0.0096 & 0.0093 & 0.0051 \\
      Luminosity              & 0.0003 & 0.0005 & 0.0002 & 0.0002 & 0.0005 & 0.0005 & 0.0000  \\
      Pre-selection           & 0.0009 & 0.0012 & 0.0021 & 0.0014 & 0.0018 & 0.0021 & 0.0018 \\
      Detector response       & 0.0064 & 0.0012 & 0.0046 & 0.0075 & 0.0177 & 0.0104 & 0.0007 \\
      c background            & 0.0089 & 0.0127 & 0.0077 & 0.0087 & 0.0144 & 0.0137 & 0.0041 \\
      uds background          & 0.0012 & 0.0025 & 0.0009 & 0.0018 & 0.0035 & 0.0027 & 0.0006 \\
      Jet charge              & 0.0627 & 0.1030 & 0.0381 & 0.1109 & 0.1317 & 0.0732 & 0.0497 \\
      b modeling :           & & & & & & & \\
      Hadron fractions         & 0.0023 & 0.0035 & 0.0014 & 0.0038 & 0.0045 & 0.0047 & 0.0016 \\
      Leptonic branching ratio & 0.0028 & 0.0046 & 0.0015 & 0.0052& 0.0057 & 0.0051 & 0.0024 \\
      Multiplicity            & 0.0039 & 0.0060 & 0.0022 & 0.0066 & 0.0072 & 0.0068 & 0.0031 \\
      Mixing                  & 0.0009 & 0.0019 & 0.0006 & 0.0019 & 0.0023 & 0.0020 & 0.0090 \\
      \hline
      Total               & 0.0641 & 0.1045 & 0.0395 & 0.1122 & 0.1345 & 0.0765 & 0.0511 \\
      \hline
    \end{tabular}
  \end{center}
\end{table}

